Accurate Forgetting for All-in-One Image Restoration Model

Privacy protection has always been an ongoing topic, especially for AI. Currently, a low-cost scheme called Machine Unlearning forgets the private data remembered in the model. Specifically, given a private dataset and a trained neural network, we need to use e.g. pruning, fine-tuning, and gradient ascent to remove the influence of the private dataset on the neural network. Inspired by this, we try to use this concept to bridge the gap between the fields of image restoration and security, creating a new research idea. We propose the scene for the All-In-One model (a neural network that restores a wide range of degraded information), where a given dataset such as haze, or rain, is private and needs to be eliminated from the influence of it on the trained model. Notably, we find great challenges in this task to remove the influence of sensitive data while ensuring that the overall model performance remains robust, which is akin to directing a symphony orchestra without specific instruments while keeping the playing soothing. Here we explore a simple but effective approach: Instance-wise Unlearning through the use of adversarial examples and gradient ascent techniques. Our approach is a low-cost solution compared to the strategy of retraining the model from scratch, where the gradient ascent trick forgets the specified data and the performance of the adversarial sample maintenance model is robust. Through extensive experimentation on two popular unified image restoration models, we show that our approach effectively preserves knowledge of remaining data while unlearning a given degradation type.

==> sections/discussion.tex <==


% \begin{figure}[t]
% % \setlength{\abovecaptionskip}{-0.in}
% % \setlength{\belowcaptionskip}{0.in}
% \centering
% \begin{subfigure}{0.245\linewidth}
%     % \centering
%     \includegraphics[width=1.\linewidth]{figs/training_curve11.pdf}
%     \caption{}
%     \label{fig:uir_curve1}
% \end{subfigure}
% \begin{subfigure}{0.245\linewidth}
%     \centering
%     \includegraphics[width=1.\linewidth]{figs/training_curve2.pdf}
%     \caption{}
%     \label{fig:uir_curve2}
% \end{subfigure}
% \begin{subfigure}{0.245\linewidth}
%     \centering
%     \includegraphics[width=1.\linewidth]{figs/training_curve3.pdf}
%     \caption{}
%     \label{fig:uir_curve3}
% \end{subfigure}
% \begin{subfigure}{0.245\linewidth}
%     \centering
%     \includegraphics[width=1.\linewidth]{figs/training_curve4.pdf}
%     \caption{}
%     \label{fig:uir_curve4}
% \end{subfigure}
% \caption{Training curves of different settings on the \emph{unified} image restoration task.}
% \label{fig:cmp_uir_curve}
% \end{figure}



\section{Discussion and Analysis}
In this section, we explore the effectiveness of integrating different embeddings from DA-CLIP into image restoration models and also analyze the influence of training patch sizes. 
% After that, we further discuss the limitations of our approach and potential future work in more detail.


% \subsection{Effectiveness of Embeddings from DA-CLIP}

We have two types of embeddings from the DA-CLIP: HQ content embedding and degradation embedding. The former is obtained from the image encoder and used for improving general image restoration performance, whereas the latter is predicted by the controller and leveraged to classify the image degradation type for unified image restoration. To verify their effectiveness, we train the baseline model with different embedding settings. As can be observed in~\Figref{fig:uir_curve1}, separately applying either the degradation embedding or the HQ content embedding improves the performance. Moreover, the performance is further improved by applying both embeddings in combination.

\begin{wrapfigure}{R}{0.3\textwidth}
\setlength{\belowcaptionskip}{-0.2in}
    \centering
    \includegraphics[width=.95\linewidth]{figs/training_curve51.pdf}
    \caption{Training curves of baseline models with DA-CLIP and OpenAI CLIP on the \emph{degradation-specific} task.}
    \label{fig:training_curve_rainy}
\end{wrapfigure}

We also compare with the model that integrates image embeddings from OpenAI CLIP~\citep{radford2021learning} into the baseline for both degradation-specific (e.g., image deraining) and unified image restoration tasks, as shown in \Figref{fig:training_curve_rainy} and \Figref{fig:uir_curve2}. We observe that both embeddings lead to better performance for the image deraining task while the model with our DA-CLIP achieves significantly higher performance overall training process. Moreover, only using content embedding from OpenAI CLIP can't make obvious improvements for unified image restoration, demonstrating the importance of controller and the corresponding degradation embeddings.

Moreover, we notice that the text encoder can also be involved in unified image restoration by giving true text degradation labels and then performing as a non-blind approach. We verify this idea and compare it with our blind approach (using predicted image degradation embedding) in~\Figref{fig:uir_curve3}. Surprisingly, we found that our blind model achieves similar performance to that with true degradation labels. That means our controller predicts highly accurate degradation types for all images.

Intuitively, large patch sizes always contain more semantic information that might be important for guiding image restoration. We explore this property by training our model with two different patch sizes on the unified image restoration task. As shown in~\Figref{fig:uir_curve4}, increasing the patch size from $128 \times 128$ to $256 \times 256$ improves the training process, which is consistent with our conjecture.





==> sections/related_work.tex <==
\section{Related Work}

Text text text... \hl{TODO!}

\hl{Combine this with a Background section, put after the Introduction?}
